Charting Visual Impression of Robot Hands

A wide variety of robotic hands have been designed to date. Yet, we do not know how users perceive these hands and feel about interacting with them. To inform hand design for social robots, we compiled a dataset of 73 robot hands and ran an online study, in which 160 users rated their impressions of the hands using 17 rating scales. Next, we developed 17 regression models that can predict user ratings (e.g., humanlike) from the design features of the hands (e.g., number of fingers). The models have less than a 10-point error in predicting the user ratings on a 0-100 scale. The shape of the fingertips, color scheme, and size of the hands influence the user ratings the most. We present simple guidelines to improve user impression of robot hands and outline remaining questions for future work.

==> table-pca.tex <==
\begin{table}[t]
\centering
  \caption{\hsE{Principal components loading matrix after Varimax rotation. Loadings above 0.5 are in bold.}}% Six rating scales that had high multicolinearity with the other scales were removed from the analysis (Friendly, Intelligent, Trustworthy, Be Touched, To Touch, Handover)~\cite{}.}}
  \label{tab:pca}
  \small{
  \begin{tabular}{lcccc}
    % \cline{2-5}
    \hline
     \cellcolor{MedGray}\textbf{Rating Scales}& \cellcolor{MedGray}\textbf{PC1} & \cellcolor{MedGray}\textbf{PC2} & 
     \cellcolor{MedGray}\textbf{PC3}\\
      \cellcolor{MedGray}\textbf{}& \cellcolor{MedGray}\textbf{Comfort} & \cellcolor{MedGray}\textbf{Interest} & 
      \cellcolor{MedGray}\textbf{Masculinity}\\
    \hline
    \multicolumn{1}{l}{To Touch} & \textbf{.96} & .16 & .06\\
    % \hline
    \multicolumn{1}{l}{Be Touched} & \textbf{.95} & .21 & -.06\\
    % \hline
    \multicolumn{1}{l}{Friendly} & \textbf{.94} & .19 & .20\\
    % \hline
    \multicolumn{1}{l}{Safe} & \textbf{.91} & .06 & -.21\\
    % \hline
    \multicolumn{1}{l}{Happy} & \textbf{.90} &	.34 & -.07\\
    % \hline
    \multicolumn{1}{l}{Trustworthy} & \textbf{.88} & .38 & .19\\
    % \hline
    \multicolumn{1}{l}{Nice} & \textbf{.87} & .21 & .16\\
    % \hline
    \multicolumn{1}{l}{Nearby} & \textbf{.86} & .34 & .31\\
    % \hline
    \multicolumn{1}{l}{Handover} & \textbf{.84} & .36 & .33\\
    % \hline
    \multicolumn{1}{l}{Dominant} & \textbf{.66} & -.23 & -.25\\
    % \hline
    \multicolumn{1}{l}{Interesting} & .30 & \textbf{.82} & .22\\
    % \hline
    \multicolumn{1}{l}{Excited} & -.07 & \textbf{.82} & .11\\
    % \hline
    \multicolumn{1}{l}{Intelligent} & \textbf{.51} & \textbf{.70} & .42\\
    % \hline
    \multicolumn{1}{l}{Capable} & .41 & \textbf{.66} & \textbf{.56}\\
    % \hline
    \multicolumn{1}{l}{Humanlike} & .49 & \textbf{.64} & -.24\\
    % \hline
    \multicolumn{1}{l}{Feminine} & .26 & -.04 & \textbf{-.90}\\
    % \hline
    \multicolumn{1}{l}{Mature} & .09 & \textbf{.54} & \textbf{.74}\\
    \hline
    \multicolumn{1}{l}{\textbf{Eigenvalue}}& 10.16 & 3.41 & 1.07\\
    \multicolumn{1}{l}{\textbf{\% Variance}}& 59.75 & 20.08 & 6.30\\
    % \multicolumn{1}{l}{\textbf{Subscale Cronbach's $\alpha$}}&&\\
    \hline
  \end{tabular}
  }
\end{table}

% \begin{table}[t]
%   \caption{Loadings of the 17 ratings on the four PCA dimensions. Humanlikeness has the highest loadings on D1 and D3. Maturity and Interestingness have the highest loadings on D2 and D4 respectively.}
%   \label{tab:pca}
%   \begin{tabular}{lcccc}
%     % \cline{2-5}
%     \hline
%      \cellcolor{MedGray}\textbf{Perceptual Attributes}& \begin{tabular}{@{}c@{}}\cellcolor{MedGray}\textbf{D1}\end{tabular} & \begin{tabular}{@{}c@{}}\cellcolor{MedGray}\textbf{D2}\end{tabular} & \cellcolor{MedGray}\textbf{D3} & \begin{tabular}{@{}c@{}}\cellcolor{MedGray}\textbf{D4}\end{tabular} \\
%     \hline
%     \multicolumn{1}{l}{Humanlike} & \textbf{0.44}	& -0.21 & \textbf{0.81} &	-0.25\\
%     % \hline
%     \multicolumn{1}{l}{Nice} & 0.27 & -0.12 & -0.23 & -0.26\\
%     % \hline
%     \multicolumn{1}{l}{Interesting} & 0.23 & 0.21 & 0.11 & \textbf{0.61}\\
%     % \hline
%     \multicolumn{1}{l}{Capable} & \textbf{0.34} & \textbf{0.39} & -0.06 &	0.11\\
%     % \hline
%     \multicolumn{1}{l}{Safe} & 0.19 &	-0.26 & -0.12 & -0.07\\
%     \hline
%     \multicolumn{1}{l}{Feminine} & 0.00 & \textbf{-0.38} &	0.16 & \textbf{0.37}\\
%     % \hline
%     \multicolumn{1}{l}{Mature} & 0.21 & \textbf{0.52} & 0.02 & \textbf{-0.37}\\
%     % \hline
%     \multicolumn{1}{l}{Friendly} & 0.24 & -0.28 & -0.15 &	0.06\\
%     % \hline
%     \multicolumn{1}{l}{Intelligent} & \textbf{0.31} & 0.24 &	-0.02 &	0.21\\
%     % \hline
%     \multicolumn{1}{l}{Trustworthy} & 0.24 & -0.05 & -0.18 & 0.05\\
%     \hline
%     \multicolumn{1}{l}{Happy} & 0.22 & -0.15 &	-0.12 &	0.11\\
%     % \hline
%     \multicolumn{1}{l}{Excited} & 0.07 & 0.14 & 0.1 & \textbf{0.35}\\
%     % \hline
%     \multicolumn{1}{l}{Dominant} & 0.04 & -0.12 & -0.11 & 0.06\\
%     \hline
%     \multicolumn{1}{l}{Comfort to Be Touched} & 0.23 & -0.19 & -0.16 &	0.01\\
%     % \hline
%     \multicolumn{1}{l}{Comfort to Touch} & 0.21 &	-0.15 & -0.22 & -0.03\\
%     % \hline
%     \multicolumn{1}{l}{Comfort to Do Handover} & 0.25 & 0.00 & -0.18 & -0.1\\
%     % \hline
%     \multicolumn{1}{l}{Comfort to Be Nearby} & 0.24 & -0.01 & -0.18 & -0.08\\
%     \hline
%   \end{tabular}
% \end{table}
